XAIport: A Service Framework for the Early Adoption of XAI in AI Model Development

In this study, we propose the early adoption of Explainable AI (XAI) with a focus on three properties: Quality of explanation, the explanation summaries should be consistent across multiple XAI methods; Architectural Compatibility, for effective integration in XAI, the architecture styles of both the XAI methods and the models to be explained must be compatible with the framework; Configurable operations, XAI explanations are operable, akin to machine learning operations. Thus, an explanation for AI models should be reproducible and tractable to be trustworthy. We present XAIport, a framework of XAI microservices encapsulated into Open APIs to deliver early explanations as observation for learning model quality assurance. XAIport enables configurable XAI operations along with machine learning development. We quantify the operational costs of incorporating XAI with three cloud computer vision services on Microsoft Azure Cognitive Services, Google Cloud Vertex AI, and Amazon Rekognition. Our findings show comparable operational costs between XAI and traditional machine learning, with XAIport significantly improving both cloud AI model performance and explanation stability.

==> Sections/images/4-cost_evaluation.tex <==
\section{Deployment and Assessing the Overhead: Costs and Resource Consumption in XAI-Integrated MLOps[2 pages]}

Integrating XAI in MLOps brings a host of benefits, but it is crucial to consider the associated costs and resource implications. The overheads introduced by XAI include increased computational demand, resource utilization, energy expenditure, and operational costs. This section provides a comprehensive analysis of these factors.



XAI methods, particularly post-hoc techniques, require additional processing power and computational time, thereby increasing the computational burden. \cite{rudin2019stop}.

The adoption of XAI also impacts various resources. Hardware-wise, the CPU, memory, and GPU requirements may rise to accommodate additional XAI processes. Software dependencies and libraries needed for XAI could add complexity to the software stack. Furthermore, human resources are needed to manage, tune, and troubleshoot XAI integrated models, which could strain teams and operations \cite{xaiprocess}.
Here we statistical analysis both computational overhead and operation overhead.

\subsection{Analysis of the computational overhead}

Energy consumption is an essential yet often overlooked aspect of XAI implementation. The increased computational burden that comes with XAI integration results in higher energy use, contributing to the overall costs and environmental impact of the system \cite{strubell2020energy}.


\subsubsection{Experiment Design}

The experiment design involved utilizing Microsoft's Azure Cognitive Services, Google's Vertex AI, and Amazon's Rekognition as the cloud AI services, alongside the integration of the proposed XAI service. The models trained using the ImageNet dataset with fifty distinct labels were assessed.

Three metrics - Precision, Recall, and F1-score - were employed to analyze the model's learning performance. Two advanced data augmentation strategies, namely CutMix and PuzzleMix, were incorporated in the training process to investigate their impacts on the model's performance and interpretability.

Additionally, different XAI methods, including Grad-CAM, Grad-CAM++, XGrad-CAM, Layer-CAM, and Eigen-CAM, were employed to produce visual explanations for the AI model's decision-making.

\subsubsection{Execution and Challenges}

Executing the experiment involved applying the designed XAI service to the chosen cloud AI services, then performing rigorous validation and statistical analyses to assess the models' performance.

The challenges encountered in the process included limited functionality and evaluation metrics provided by the cloud AI services, which constrained the interpretability of the AI models, especially when data augmentation strategies were used. To overcome this, the proposed XAI service was integrated, enabling users to define their test sets and offering a broader range of evaluation metrics, which provided a more in-depth understanding of the models' performance and interpretability.


\subsubsection{Results Presentation}

The results of the experiments are visually presented in Figure~\ref{fig:timeratio}. The stacked bar charts represent the proportion of time consumed by each operation in the total computational process. The operations are color-coded for easy identification. It is notable that each operation's duration contributes significantly to the overall computation time, highlighting the cost of interpretability.

In all cloud AI services - Azure Cognitive Services, Google Vertex AI, and Amazon Rekognition - the most time-consuming operation was EigenCAM. The time consumption for EigenCAM was significantly higher than other methods, such as Grad-CAM, Grad-CAM++, Layer-CAM, and XGrad-CAM, indicating the complexity and computational demand of this method.

The model's prediction time was relatively stable across all operations and cloud services. Among the cloud AI services, Azure Cognitive Services showed the least time consumption in most of the combinations, followed by Google Vertex AI, while Amazon Rekognition showed the highest time consumption.

Data uploading and stability computing time remained constant across all combinations. However, it is noteworthy that stability computing takes up a considerable portion of the total time, which calls for optimization efforts.

By offering a visual comparison between different combinations of operations, the diagram provides a clearer understanding of the trade-offs involved in choosing specific XAI methods and cloud AI services.
\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{Sections/images/timeratio.png}
\caption{Time ratio of different operations in various combinations across Azure Cognitive Services, Google Vertex AI, and Amazon Rekognition.}
\label{fig:timeratio}
\end{figure}

We evaluated energy consumption during computation, focusing on the computational resources used by each method. This is particularly important for real-time applications and large-scale data processing tasks.
For client-side operational overhead, it is paramount to integrate the API into the microservice for invocation by the system. Given the architecture and API design, users need to prepare the invocation methods for either the AI cloud services or their own deployed AI models, which can then be coupled with the microservice. 
%Considering the operational overhead of the XAI methods, we assess the execution energy consumed for computation. The computational resources used by each method are critical factors, especially for real-time applications and large-scale data processing tasks.

We performed the XAI methods on an identical infrastructure to ensure fairness in comparison. We analyzed the bottlenecks and overhead of the XAI service system by collecting data on microservice response time and computational resource consumption during experiments. The analysis was performed by reviewing the code and conducting local tests, which revealed that the software's resource usage linearly increased with the workload.
Table \ref{tab:EnergyConsumption} summarizes the average computational resources used by each XAI method and associated microservices per data sample.

\begin{table}[htbp]
  \caption{Energy consumption for the XAI service system (average per data sample) in $10^-6$ kWh}
  \label{tab:EnergyConsumption}
  \begin{adjustbox}{width=\linewidth, center}
  \begin{tabular}{lcccc}
    \toprule
    \textbf{Microservices} & \textbf{\textit{CPU Energy}} &  \textbf{\textit{GPU Energy}} &  \textbf{\textit{RAM Energy}} &  \textbf{\textit{Energy Consumed}} \\ 
    \midrule
    Data process &  3.60 & N/A & 0.08 & 3.68 \\
    Resnet model &  1.61 & 3.77 & 0.02 & 5.39 \\
    Densenet model &  0.38 & 0.89 & 0.02 & 1.28 \\
    GradCAM &  8.32 & 19.50 & 0.10 & 27.91 \\
    GradCAM++ &  7.09 & 15.93 & 0.09 & 23.11 \\
    EigenCAM &  121.48 & 107.54 & 1.71 & 230.74 \\
    LayerCAM &  7.21 & 10.08 & 0.09 & 17.37 \\
    XGradCAM &  6.77 & 17.35 & 0.08 & 24.20 \\
    Evaluation &  16.32 & N/A & 0.17 & 16.49 \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \footnotesize{Note: The values in the table are multiplied by $10^6$. Energy consumption is expressed in kilowatt-hours (kWh). The CPU, GPU, and memory usage data were obtained from a local host using experimental programs, providing insights into system performance and potential optimizations.}
\end{table}







% \begin{table}[ht]
% \caption{Energy consumption for the XAI service system (average per data sample) in $10^-6$ kWh}
% \renewcommand{\arraystretch}{1.2}
% \begin{center}
% % \begin{tabular}{M{2cm} | M{1cm} M{1cm} M{1cm} M{1.5cm}}
% \hline
% \textbf{Microservices} & \textbf{\textit{CPU Energy }} &  \textbf{\textit{GPU Energy}} &  \textbf{\textit{RAM Energy}} &  \textbf{\textit{Energy Consumed}} \\ 
% \hline
% \textbf{Data process} &  3.60 & N/A & 0.08 & 3.68 \\
% \textbf{Resnet model} &  1.61 & 3.77 & 0.02 & 5.39 \\
% \textbf{Densenet model} &  0.38 & 0.89 & 0.02 & 1.28 \\
% \textbf{GradCAM } &  8.32 & 19.50 & 0.10 & 27.91 \\
% \textbf{GradCAM++ } &  7.09 & 15.93 & 0.09 & 23.11 \\
% \textbf{EigenCAM } &  121.48 & 107.54 & 1.71 & 230.74 \\
% \textbf{LayerCAM } &  7.21 & 10.08 & 0.09 & 17.37 \\
% \textbf{XGradCAM } &  6.77 & 17.35 & 0.08 & 24.20 \\
% \textbf{Evaluation} &  16.32 & N/A & 0.17 & 16.49 \\
% \hline
% \end{tabular}
% \end{center}
% \label{EnergyConsumption}
% \end{table}
% \footnotesize{Note: The values in the table are multiplied by $10^6$. Energy consumption is expressed in kilowatt-hours (kWh). The CPU, GPU, and memory usage data were obtained from a local host using experimental programs, providing insights into system performance and potential optimizations.}
% \normalsize

From Table \ref{EnergyConsumption}, we observe that Layer-CAM has the lowest computational overhead in terms of CPU and GPU usage. This suggests that Layer-CAM might be better suited for systems where compute resource availability is limited.
On the other hand, Eigen-CAM shows the highest computational resource utilization and execution time, in line with its lower performance in the prediction change and stability tests.

Overall, these results imply that there is a trade-off between the quality of the explanations, computational efficiency, and time efficiency. This indicates that the choice of the XAI method should consider the specific requirements and constraints of the application.
\subsubsection{Detailed Analysis}

The analyses revealed that data augmentation techniques significantly enhanced both model performance and interpretability. The Layer-CAM and Grad-CAM methods were most effective at providing reliable explanations for the AI model's decision-making, with few prediction changes across the test set.

Interestingly, although the Eigen-CAM method initially appeared to offer less reliable explanations, its performance significantly improved with the application of data augmentation techniques. This observation underlined the potential of data augmentation techniques to enhance the performance of XAI methods, indicating the importance of considering data augmentation not only for improving model performance but also for optimizing explanability.

\subsubsection{Implications}

The experimental results and their analysis yielded significant insights into the roles of data augmentation strategies and XAI methods in enhancing AI model performance and interpretability. The findings indicated the potential of data augmentation techniques to not only improve the performance of XAI methods but also their stability, thereby yielding more reliable explanations for model decision-making.

Moreover, the study underscored the importance of a comprehensive evaluation strategy when investigating the impact of data augmentation on AI models. The exclusive reliance on traditional performance metrics could overlook the broader influence of these techniques, especially their enhancement of model interpretability, which is crucial for creating reliable and transparent AI systems.

\subsection{Navigating the Trade-Off Between Overhead and Added Value of XAI in MLOps}

The integration of XAI in MLOps introduces additional overheads but also provides a significant increase in model interpretability and trustworthiness. While XAI techniques can require more computational resources and add complexity, they offer crucial insights into model behavior, leading to enhanced control over model decisions \cite{arrieta2020explainable, ribeiro2016should}. 


The decision to implement XAI should consider both the associated costs and the balance between these costs and the value added to the ML system \cite{strubell2020energy}. Understanding this trade-off is essential for the successful implementation of MLOps with the goal of creating more responsible, reliable, and transparent ML models. In this decision-making process, a comprehensive evaluation of both tangible and intangible factors is necessary. These include computational resources, time, model interpretability, ethical implications, and the overall impact on business and societal outcomes \cite{miller2019explanation}. 

This synthesis of cost-benefit analysis underlines the growing relevance of XAI in MLOps, positioning it as a crucial component in the responsible and effective deployment of ML systems.





==> Sections/images/backup.tex <==
%previous version
\section{XAI Early Adoption into MLOps Workflow}
In the rapidly evolving field of MLOps \cite{kreuzberger2023machine}, the adoption of XAI in the early stages allows us to align AI systems with ethical standards, enhance model reliability and trust, and enable more effective debugging and model refinement.
We explore the intersection in detail in Figure \ref{fig:earlyadoption}, which visually represents the integration of XAI in each phase of the MLOps workflow \cite{kreuzberger2023machine}.
Here, the blue-shade units are XAI operations, while the white units are operations from general machine learning.

% \subsection{Workflow Overview}
% Following the schematic representation of the MLOps architecture, our focus is to propose a structured workflow to assist machine learning researchers and practitioners who seek to incorporate XAI techniques into their projects. This is further clarified in Figure \ref{fig:XAI_in_MLOps}, which provides a step-by-step guide for the sequence of tasks in the various stages of this workflow.

% Figure \ref{fig:XAI_in_MLOps} illustrates our strategy that offers a streamlined pathway for the integration of machine learning and XAI techniques within the MLOps lifecycle. This represents our comprehensive approach, designed to facilitate the adoption of XAI operations.

\begin{figure*}[htbp]
\centerline{\includegraphics[width=1.0\linewidth]{Sections/images/Mlops pipeline.drawio.png}}
\caption{Early adoption of XAI into the MLOps Workflow}
\label{fig:earlyadoption}
\end{figure*}


% The initiation of an MLOps product starts by pinpointing a problem that can be resolved using machine learning techniques. After identifying the problem, the appropriate technologies are selected for execution \cite{sculley2015hidden}. This problem is further refined into a precise machine learning task, followed by the identification and preparation of necessary data. This data preparation involves sourcing raw data, performing initial data analysis, and ensuring accurate labeling for supervised learning \cite{bertsimas2020predictive}.

% Feature engineering is a crucial step in the machine learning pipeline, transforming raw data into a structured format ready for model consumption \cite{kuhn2013applied}. This process begins with connecting to data sources and extracting the required data. The extracted data undergoes transformation and cleaning to ensure its quality and consistency. Subsequently, the cleaned data is used to create meaningful features. Lastly, the engineered features are ingested into a designated storage system, ensuring that the raw data is transformed into usable features, thus enhancing the efficacy and accuracy of the machine learning models.

% The machine learning development process encompasses data preparation, model training, validation, and model exportation. Model training involves learning from the prepared data, adjusting model parameters, and minimizing error using techniques such as gradient descent or regularization \cite{bengio2012practical}. Validation evaluates the model's performance on unseen data, utilizing measures such as accuracy, precision, or recall, and involves hyperparameter tuning to optimize model performance. Lastly, the validated and optimized model is exported for deployment, serving as a tool for predicting or classifying new data \cite{goodfellow2016deep}.

% While metrics such as precision, recall, and F1 score provide valuable measures of a model's performance, they do not offer insights into the model's decision-making processes. 
% However, XAI offers a comprehensive understanding of the contributing factors to a model's predictions, providing a set of evaluation metrics, thereby enabling more profound insights into model performance and decision-making processes \cite{arrieta2020explainable}. Thus, XAI methods serve as critical tools for effectively understanding, evaluating, and improving machine learning models.

\subsection{The effectiveness of Post-hoc XAI Techniques}

Post-hoc XAI methods are essential tools for interpreting trained machine learning models, providing insights into the model's decision-making mechanisms \cite{xaiprocess}.

These methods encompass many techniques. For instance, Local Interpretable Model-Agnostic Explanations (LIME) are techniques providing instance-level interpretability, unraveling the reasons behind individual predictions \cite{ribeiro2016should}. Similarly, SHapley Additive exPlanations (SHAP) offer insights into the contribution of individual features to specific predictions \cite{lundberg2017unified}. Other techniques like Partial Dependence Plots (PDPs) offer a more global view of how features affect model output \cite{friedman2001greedy}.

These methods play a vital role in establishing transparency and trust in machine learning models, particularly in sensitive areas such as healthcare \cite{caruana2015intelligible,sanchez2019machine,gulshan2016development} and criminal justice \cite{kleinberg2018human}, where the stakes are high and comprehensible justifications are needed for each prediction.

In essence, post-hoc XAI methods not only enrich our understanding of complex models but also enhance their validation and improvement processes, thereby bolstering the effectiveness and trustworthiness of machine learning deployments.

\subsection{Benefits of XAI in MLOps}
The integration of Explainable Artificial Intelligence (XAI) into Machine Learning Operations (MLOps) provides a substantial number of benefits, significantly enhancing the transparency, reliability, and effectiveness of machine learning deployments.

The primary benefits of XAI is the increased transparency and trust in machine learning models. Often, machine learning models can be seen as "black-boxes" due to their complex internal mechanisms, which can lead to mistrust and misuse of models, especially in critical areas such as healthcare \cite{caruana2015intelligible,sanchez2019machine}. XAI methods can help mitigate these issues by providing interpretable insights into the model's decision-making processes, enabling stakeholders to better understand and trust the model's predictions \cite{ribeiro2016should,kleinberg2018human}.

Moreover, XAI aids in the model validation and refinement process. The explanations provided by XAI methods can help to identify whether the model is making predictions based on sensible features, or if it's relying on irrelevant or biased features. This not only aids in verifying the model's performance but also in improving the model by adjusting or eliminating such unwanted dependencies \cite{lundberg2017unified,friedman2001greedy}.

Lastly, XAI increases the accessibility and adaptability of machine learning models. With XAI, not only can data scientists understand the model's workings, but so can non-expert stakeholders, such as business managers or auditors \cite{miller2019explanation}. This wider understanding can lead to better-informed decision-making processes, promoting the broader adoption of machine learning solutions across various domains.

Therefore, the adoption of XAI in MLOps signifies a substantial advancement toward more understandable, trustworthy, and effective use of machine learning. It reinforces the potential of machine learning solutions in various industries, bridging the gap between the complex world of machine learning and its practical, understandable application \cite{arrieta2020explainable}.

\subsection{Identification of Scenarios}
improve
Cloud Services
Operations,envoke in framework
cost operations
devops overhead.
MOre analysis per senarios on cost operations.
1 understand cloud AI
2 keep costs low
New operation cost.
threads of validity: more user based validation.
Learning performance, describe discovery summary first. Alibaba Cloud 

\subsection{Assessing the Cloud AI Services using XAI}

Understanding the importance and utility of XAI in MLOps can be emphasized further by identifying specific use-case scenarios where the interpretability of machine learning models becomes indispensable.

In the realm of computer vision, one can consider the application of machine learning in healthcare, specifically in diagnosing diseases from medical imagery. it is crucial for healthcare professionals to understand the rationale behind these diagnoses to ensure trust in the system \cite{caruana2015intelligible,sanchez2019machine,gulshan2016development}. XAI can provide these much-needed insights, thereby assisting doctors to confirm that the models are making sensible predictions.

Moreover, machine learning models are extensively used in safety-critical domains such as autonomous driving. Here, convolutional neural networks (CNNs) are employed for tasks like object detection and semantic segmentation, which are integral for vehicle perception \cite{bojarski2016end}. XAI methods \cite{selvaraju2017grad} can provide saliency map for the CNN-based model.

In the realm of tabular data-based machine learning, for instance, consider a model trained on the Adult dataset, which includes features such as age, education, marital status, and occupation. When the model makes a prediction of incomes, SHAP \cite{lundberg2017unified} values are computed for each feature, illustrating the contribution of each towards the specific prediction.

The application of SHAP \cite{lundberg2017unified} in this context demystifies the decision-making process of the model, thus enhancing interpretability. This not only boosts our understanding of the model's outputs but also facilitates an evaluation of the model's fairness and reliability. Therefore, SHAP values play a crucial role in ensuring transparency and fostering trust in machine learning models that are based on tabular data.

These scenarios elucidate the widespread applicability and crucial role of XAI in MLOps. By offering interpretable insights into machine learning models, XAI assures that these models are not only high-performing but also transparent, trustworthy, and prepared for real-world deployment.


==> Sections/implementation.tex <==
\section{Design the Phases of XAI Early Adoption into MLOps Workflow}
In the rapidly evolving field of MLOps \cite{kreuzberger2023machine}, the proactivity in integrating XAI from the onset allows us to design AI systems in line with ethical standards, improve model trustworthiness and reliability, and facilitate efficient debugging and model tuning.

\begin{figure*}[ht]
\centerline{\includegraphics[width=1.0\linewidth]{Sections/images/Mlops pipeline.drawio.png}}
\caption{Early adoption of XAI into the MLOps Workflow}
\label{fig:earlyadoption}
\end{figure*}

The representation in Figure \ref{fig:earlyadoption} describes the integration of XAI at different phases of the MLOps pipeline \cite{kreuzberger2023machine}. The distinction between XAI operations (blue-shaded units) and traditional MLOps components (white units) offers a comprehensive view of the workflow. The details description follows:


\textbf{Phase 1: Requirement and Responsibility Planning} \\
 This phase encompasses three main sub-components: Requirements Definition, Responsible Requirements Analysis, and Risk Assessment.
 
\textbf{\textit{Requirements Definition.}} Defining system requirements, use cases, and constraints is a standard procedure in ML workflow \cite{kreuzberger2023machine}. An article by Habibullah et al. \cite{Habibullah2022NonFunctionalRF} consolidates a list of requirements for ML systems, indicating that activities related to requirement analysis and specification are generally conducted in the early phases of development.

\textbf{\textit{Responsible Requirements Analysis.(XAI)}} Ethics, fairness, explainability, and so on are on the list of the important non-functional requirements of ML \cite{Habibullah2022NonFunctionalRF}. These are requirements that need to be conducted at the initial phase of development. 
The data provenance that describes the origins and processing of data can help improve the fairness, accountability, transparency, and explainability (FATE) goals of ML systems \cite{Werder2022EstablishingDP}. 

\textbf{\textit{Risk Assessment.(XAI)}} Traditional risk assessment often relies on quantifying loss by its probability \cite{aven2011some}. Recent advancements include Meskauskas' XAI-based toolkit for risk evaluation \cite{Meskauskas2022AboutTN}, as well as work on XAI-based vulnerability detection \cite{Nguyen2021HumanintheLoopXV}. XAI is pivotal in assessing risks and vulnerabilities, helping to flag models that may yield unpredictable or misleading results \cite{Meskauskas2022AboutTN}.

By proactively addressing responsible requirements and risks at the early stages of the MLOps process, we ensure alignment with ethical standards and lay the foundation for creating trustworthy and reliable AI systems \cite{xaiprocess}.

\textbf{Phase 2: Data Management} \\
XAI improves data quality by eliminating biases and facilitating data augmentation.

\textbf{\textit{Data Collection, Cleaning, and Labeling.}} In conventional ML workflows, Data Collection, Cleaning, and Labeling primarily ensure that the collected data are fit for model training \cite{whang2020data}. However, these steps often overlook the biases that can inadvertently be introduced, thereby affecting the model's fairness and reliability.

\textbf{\textit{Data Bias Elimination.(XAI)}}
Leveraging XAI techniques allows for the identification and mitigation of implicit biases in the dataset, thus training the AI model on more balanced and fair data \cite{arrieta2020explainable}. The effective use of feature attribution methods, assessed through metrics like the "Focus" score, can add another layer of reliability to the model by objectively gauging the coherency of these explanations \cite{duart2022}.

\textbf{\textit{Data Augmentation.(XAI)}} It aims to enhance the data quality and improve model generalizability. By leveraging techniques such as cutmix \cite{cutmix} and puzzlemix \cite{puzzlemix}, we can enrich the training dataset without further collection.

\textbf{Phase 3: Feature Handling} \\
Preparing features is an essential but labor-intensive element in ML implementations \cite{Bengio}. This phase comprises three sub-components: Feature explanation, Feature Engineering, and Feature Selection.

\textbf{\textit{Feature Explanation.(XAI)}} Also known as Explanation of Feature Importance, it provides why certain features are pivotal for model decision-making \cite{lundberg2017unified}. The work of XAI process \cite{xaiprocess} shows three case studies that obtain feature importance explanation by feature masking methods and feature mutation methods. 

\textbf{\textit{Feature Engineering and Selection.}} These are critical processes in the development of ML models \cite{Bengio}. While feature engineering focuses on transforming or creating new variables to better represent the problem, feature selection is concerned with choosing the most relevant variables to reduce dimensionality and improve performance.
feature selection with explanation results reduces irrelevant variables from the model \cite{zacharias2022designing}. This helps simplify the model structure, makes it more interpretable, and can lead to a decrease in training and prediction time. 

\textbf{Phase 4: Model Development} \\
The three stages are model selection, training, and hyperparameter tuning. Model selection involves choosing an appropriate algorithm based on the problem's characteristics and data distribution. Subsequently, model training is executed to learn the data, optimizing model parameters to minimize a specific loss function. Lastly, hyperparameter tuning refines the model by optimizing predefined settings that guide the training process \cite{Turner2021BayesianOI}. 

While XAI methods may not directly participate in these stages, the model selection can be guided by requirements for responsibility and the explanation result. There are two factors: the inherent interpretability of the selected algorithm \cite{rudin2019stop} and the presence of model-specific explanatory methods \cite{xaiprocess}. Hence, XAI can significantly influence configuration choice in model development.

\textbf{Phase 5: Model Validation and Explanation} \\
In ML workflow, the model validation check is iteratively repeated until a good result has been achieved \cite{kreuzberger2023machine}. We add model explanation and XAI evaluation into this phase. 

\textbf{\textit{Model Validation.}}
Validation is often constrained to performance metrics, such as precision, recall, and F1 score \cite{Zuhair2022AnalysisOB}. These metrics offer a quantitative measure of the model's performance but overlook the explainability requirements, especially in cloud AI services\cite{azure-cognitive-services,google_cloud_vertex_ai,aws-ai-services,Zuhair2022AnalysisOB}.

\textbf{\textit{Result Explanation.}} The explanation provides detailed insights into the model's predictions. Execute the XAI methods to get an explanation. The process for achieving this is comprehensively described in prior research \cite{xaiprocess}, which includes the fundamentals of the XAI process and case studies in different domains to demonstrate the effectiveness of result explanations.

\textbf{\textit{Explainability Evaluation.}}
XAI Evaluation is for assessing the trustworthiness of explanations. Specifically, consistency evaluation can be employed to perform statistical analyses on the explanation results \cite{xaiprocess}. The key metrics are stability and consistency \cite{xaiprocess}. These metrics provide quantifiable measures for assessing the explanations.

\textbf{Phase 6: Deployment} \\
The final phase focuses on the production operation of ML models. What sets this phase apart is the incorporation of XAI techniques to assure transparency in production.

\textbf{\textit{Deployment Operation.}}
Incorporating a monitoring solution equipped with visualization capabilities is pivotal for ML deployment operations. Such visualization tools facilitate an intuitive comprehension of the model. XAI taxonomy lists many visualization capabilities for the model \cite{xaiprocess}.

\textbf{\textit{Production Transparency Assurance.(XAI)}}
XAI is crucial in ensuring transparency for AI services deployed in cloud platforms. Utilizing Open API XAI Service within the ML production allows for traceable explanations and evaluations of deployed models. Additionally, We work on the XAI service to collect provenance data, creating a transparent record of model operations.

To encapsulate, prioritizing XAI from the early stages in the MLOps workflow doesn't merely cater to ethical and compliance mandates; it essentially elevates the AI system's efficacy, reliability, and societal acceptance.






==> Sections/relatedworks.tex <==
\section{Related Works}
This section explores the urgent need for XAI in domains and the indispensable role of XAI in quality assurance and specialized models. 


% \subsection{The Pressing Needs for XAI in Specific Domains}
% AI models are being increasingly deployed across various industries, leading to an urgent need for XAI~\cite{adadi2018peeking}. In critical domains such as healthcare, finance, and legal systems, the understanding of AI behavior is crucial to prevent errors or biases with potentially profound consequences~\cite{arrieta2020explainable, pawar2020incorporating, ohana2021explainable}. In healthcare, the need for XAI is especially pronounced due to the growing reliance on AI technologies~\cite{Lambin2017RadiomicsTB}. Understanding AI's decisions and implications is necessary for compliance with legal and ethical protocols, demonstrating the essential role of XAI in ensuring transparency and accountability across real-world domains.


% A literature survey ~\cite{sheu2022survey}  presents a comprehensive overview of medical XAI, including model enhancements, evaluation techniques, case studies, open-box architecture, and openly available medical datasets. Significant differences between traditional AI and XAI methods are highlighted.
% Besides, In the industrial sphere, the integration of XAI highlights a semantic model approach that is vital for manufacturing \cite{ahmed2022artificial}. The pervasiveness of XAI across these diverse sectors underscores its importance in contributing to AI systems.

% As the complexity and sophistication of deep learning models increase, so does the need for explainability \cite{adadi2018peeking}. Explainability allows for a better understanding of model behavior, facilitates trust, and promotes responsible AI use \cite{arrieta2020explainable}. 

\subsection{ML workflow and Its Relationship to XAI}
%challenges
Integrating XAI into the ML workflow presents distinct challenges and increases the complexity of the MLOps pipeline due to additional operational steps and computational resources required for XAI~\cite{xaiprocess}. The existing literature reveals several gaps, notably a deficiency in the comprehensive exploration of the feasibility, impacts, tangible benefits, and increased resource requirements of implementing XAI in ML workflow. 
%The early adoption of XAI, a primary focus of our research, remains an underexplored domain with potentially significant benefits. Recognizing this deficiency, our research aims to bridge these gaps, proposing a structured methodology for the early adoption of XAI in developing ML models within the MLOps framework, ultimately optimizing the MLOps process~\cite{kreuzberger2023machine}.

%The early integration of XAI into MLOps stands as a promising approach to advance the understanding of model predictions, uncovering essential features and decision-making processes~\cite{lundberg2017unified}. The need for early comprehension of the model and the growing demand for interpretability necessitates a more strategic exploration of incorporating XAI into MLOps from the outset. Our research contributes to this area by proposing a structured and scalable methodology for the early adoption of XAI. This not only optimizes the MLOps process but also enriches the collective understanding of the real-world implications, costs, and the necessary framework for integrating XAI into MLOps~\cite{kreuzberger2023machine}.

% Integrating XAI into ML workflow presents distinct challenges. The complexity of the MLOps pipeline tends to increase due to the additional operational steps and computational resources required for XAI \cite{xaiprocess}. Moreover, the review of the existing literature highlights several gaps. There is a lack of thorough research on the feasibility, impacts, and benefits, along with the associated increases in resources of implementing XAI in MLOps. The operational and computational implications of early adoption of XAI in MLOps, a primary focus of our research, are not well explored and understood in the existing literature.

% The early integration of XAI into MLOps can enhance the understanding of model predictions, finding the important feature that the model is concerned \cite{lundberg2017unified}. The need for early comprehension of the model and the growing demand for interpretability necessitates the exploration of incorporating XAI into MLOps from the outset. Our research aims to bridge this gap, proposing a structured methodology for the early adoption of XAI in developing ML models within the MLOps framework, ultimately optimizing the MLOps \cite{kreuzberger2023machine}. Our research aims to provide a comprehensive understanding of the real-world implications, costs, and the necessary framework for integrating XAI into MLOps.


% The synergistic integration of XAI into ML Operations is a complex task marked by distinct challenges. The complexity of the MLOps pipeline tends to increase due to the additional operational steps and computational resources required for XAI \cite{xaiprocess}. Moreover, the review of the existing literature highlights several gaps. Notably, there exists a deficiency in the comprehensive exploration of the feasibility, impacts, and tangible benefits of implementing XAI in MLOps, considering both the technological and organizational aspects. The early adoption of XAI, a fundamental aspect of our research, remains an underexplored domain with potentially significant benefits.



% Recognizing this, the early integration of XAI into MLOps stands as a promising approach to advance the understanding of model predictions, uncovering essential features and decision-making processes. The need for early comprehension of the model and the growing demand for interpretability necessitates a more strategic exploration of incorporating XAI into MLOps from the start. Our research contributes to this space, proposing a structured and scalable methodology for the early adoption of XAI. This not only optimizes the MLOps process but also enriches the collective understanding of the real-world implications, costs, and the necessary framework for integrating XAI into MLOps \cite{kreuzberger2023machine}.

A recent study \cite{zacharias2022designing} posits that feature selection in ML development should be based on XAI findings. They outline meta-requirements, emphasizing that \textit{feature selection should champion explainability} and \textit{feature selection should satisfy predictive performance standards}. Their research employs the SHAP \cite{lundberg2017unified} XAI approach, a technique for clarifying which feature affects the model's output. 
%The authors affirm that leveraging XAI for feature selection considerably impacts model predictions, ultimately enhancing model explainability and facilitating comprehension of decision logic, even for non-specialists.

% \subsection{MLOps Quality Assurance with XAI}

% In the context of industrial applications, It is important to maintain high software quality, as it alleviates the costly process of error correction~\cite{poth2020}. Despite the noted importance, the task of evaluating, ensuring, and enhancing software quality and reliability remains fraught with challenges~\cite{Hamada2020GuidelinesFQ}.

% Guidelines for quality assurance within ML models were expounded by~\cite{Hamada2020GuidelinesFQ}, highlighting the unique characteristics of ML-based systems across various domains. This paper emphasizes the importance of implementing metrics and AI evaluation to reach the desired quality benchmarks.
% However, the analysis presented in~\cite{poth2020} explored ways to ascertain ML model quality but was limited in proposing questionnaires as the sole method. This approach overlooks the multifaceted insights that XAI can provide on the model, including but not limited to interpretability and transparency.

% XAI offers more than the explanation of prediction results; it can be employed to identify models at an early stage, providing an in-depth interpretation of complex ML models, including aspects such as feature importance and behavioral explanation.

% In a more recent contribution, \cite{weber2023applications} thoroughly reviews the deployment of XAI within the finance sector. By integrating transparent design with XAI techniques, the paper illustrates how XAI can align the outputs of AI models with regulatory and business requirements. This research underscores the significance of early risk identification and mitigation and compliance with transparency and relevant standards, particularly in the financial domain~\cite{weber2023applications} and medical domain~\cite{sheu2022survey}.



% MLOps has emerged as a crucial discipline that merges the principles of DevOps with ML, enabling a more structured, efficient, and reliable method of developing and deploying ML models \cite{kreuzberger2023machine}. With its comprehensive methodology, it streamlines the entire lifecycle of ML models, from ideation to deployment, monitoring, and continuous improvement. MLOps provides a path to scaling and managing ML models, from development to production \cite{sculley2015hidden}. However, despite its benefits, such as agility and reproducibility, the complexity and lack of interpretability in the models can present significant challenges, thereby leading to the necessity for XAI in MLOps.

% \subsection{Post hoc XAI Methods}

% As AI models become integral in various sectors, the demand for transparency and interpretability is increasingly critical, leading to the development of XAI \cite{guidotti2018survey}. XAI aims to bridge the transparency gap in AI, providing insights into complex models, and thus enhancing model interpretability, fairness, and reliability \cite{arrieta2020explainable}.

% Among the array of methods in XAI, model-agnostic approaches have gained significant attention. These methods are independent of the underlying model architecture and hence can be universally applied across different models, providing a standardized way to interpret model decisions \cite{xaiprocess}. Notable model-agnostic methods include SHAP (SHapley Additive exPlanations).

% SHAP is a unified measure of feature importance that allocates each feature's contribution to the prediction for each instance. It offers a coherent and consistent allocation scheme, as it is grounded in Shapley values from cooperative game theory, allowing for equitable attribution of feature importance \cite{lundberg2017unified}.

% Despite the advancement in XAI methods, their incorporation into the ML life cycle remains challenging because of factors such as computational burdens, the intricate nature of AI models, and the lack of standardized practices to integrate these methods into the ML workflow seamlessly.


==> Sections/workflow.tex <==




% The XAI evaluation metrics are integrated into the existing MLOps workflow, allowing for simultaneous assessment of traditional performance metrics and explainability metrics. 
% Specifically, in the model validation steps, besides the accuracy, XAI operations are also performed to produce explanations. The explanations are further evaluated with the defined metric.
% These evaluations are recorded and used as conditions for decision-making within the ML workflow, determining if a model should proceed to the next stage or be retrained.


% \subsection{Design the Phases of XAI Early Adoption into MLOps Workflow}
% The representation in Figure \ref{fig:earlyadoption} describes the integration of XAI at different phases of the MLOps pipeline \cite{kreuzberger2023machine}. The details description follows:

% \begin{figure}[ht]
% \centerline{\includegraphics[width=\linewidth]{Sections/images/MLops XAIops.png}}
% \caption{Early adoption of XAI into the MLOps Workflow}
% \label{fig:earlyadoption}
% \end{figure}

 
% \textbf{\textit{Requirements Definition.}} Defining system requirements, use cases, and constraints is a standard procedure in ML workflow \cite{kreuzberger2023machine}. An article by Habibullah et al. \cite{Habibullah2022NonFunctionalRF} consolidates a list of requirements for ML systems, indicating that activities related to requirement analysis and specification are generally conducted in the early phases of development.

% % \textbf{\textit{XAI Criterion.}} There are three key aspects of the criterion \cite{xaiprocess}. The first criterion focuses on understanding the underlying mechanism of the AI model, contributing to model transparency and decision support \cite{Binns_2018,bussone2015role}. The second emphasizes the relationship between input features and output, examining feature influence and causality \cite{lundberg2017unified}. The third criterion addresses fairness, bias, privacy awareness, and transferability, aimed at identifying issues \cite{Chouldechova2017FairPW}. 

% \textbf{\textit{Data Collection.}} In conventional ML workflows, Data Collection, Cleaning, and Labeling primarily ensure that the collected data are fit for model training \cite{whang2020data}. However, these steps often overlook the biases that can inadvertently be introduced, thereby affecting the model's fairness and reliability.

% \textbf{\textit{Data Preprocessing.}} It aims to enhance the data quality and improve model generalizability. By leveraging techniques such as cutmix \cite{cutmix} and puzzlemix \cite{puzzlemix}, we can enrich the training dataset without further collection.


% \textbf{\textit{Feature Engineering.}} These are critical processes in the development of ML models \cite{Bengio}. While feature engineering focuses on transforming or creating new variables to better represent the problem, feature selection is concerned with choosing the most relevant variables to reduce dimensionality and improve performance.
% feature selection with explanation results reduces irrelevant variables from the model \cite{zacharias2022designing}. This helps simplify the model structure, makes it more interpretable, and can lead to a decrease in training and prediction time. 

% \textbf{\textit{Feature Contribution Explanation.}} Also known as Feature Importance, it provides why certain features are pivotal for model decision-making \cite{lundberg2017unified}. The work of XAI process \cite{xaiprocess} shows three case studies that obtain feature importance explanation by feature masking methods and feature mutation methods. 


% \textbf{\textit{Model Quality Assurance.}}
% Validation is often constrained to performance metrics, such as precision, recall, and F1 score \cite{Zuhair2022AnalysisOB}. These metrics offer a quantitative measure of the model's performance but overlook the explainability requirements, especially in cloud AI services\cite{azure-cognitive-services,google_cloud_vertex_ai,aws-ai-services,Zuhair2022AnalysisOB}.


% \textbf{\textit{Consistency Evaluation.}}
% XAI Evaluation is for assessing the trustworthiness of explanations. Specifically, consistency evaluation can be employed to perform statistical analyses on the explanation results \cite{xaiprocess}. The key metrics are stability and consistency \cite{xaiprocess}. These metrics provide quantifiable measures for assessing the explanations.


% \textbf{\textit{Deployment.}}
% Incorporating a monitoring solution equipped with visualization capabilities is pivotal for ML deployment operations. Such visualization tools facilitate an intuitive comprehension of the model. XAI taxonomy lists many visualization capabilities for the model \cite{xaiprocess}.

% To encapsulate, prioritizing XAI from the early stages in the MLOps workflow doesn't merely cater to ethical and compliance mandates; it essentially elevates the AI system's efficacy, reliability, and societal acceptance.





